Multiparty Session Actors

Actor coordination armoured with a suitable protocol description language has been a pressing problem in the actors community. We study the applicability of multiparty session type (MPST) protocols for verification of actor programs. We incorporate sessions to actors by introducing minimum additions to the model such as the notion of actor roles and protocol mailbox. The framework uses Scribble, which is a protocol description language based on multiparty session types. Our programming model supports actor-like syntax and runtime verification mechanism guaranteeing type-safety and progress of the communicating entities. An actor can implement multiple roles in a similar way as an object can implement multiple interfaces. Multiple roles allow for inter-concurrency in a single actor still preserving its progress property. We demonstrate our framework by designing and implementing a session actor library in Python and its runtime verification mechanism.

==> eptcsdata.tex <==
\providecommand{\firstpage}{32}
\providecommand{\publicationstatus}{Alastair F. Donaldson, Vasco Vasconcelos (Eds.): Proceedings\\ of the 7th Workshop on Programming Language Approaches\\ to Concurrency and Communication-cEntric Software (PLACES 2014)\\
EPTCS 155, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.155.5}{10.4204/EPTCS.155.5}}
\pdfoutput=1

